Recovery Guarantees of Unsupervised Neural Networks for Inverse Problems trained with Gradient Descent

Advanced machine learning methods, and more prominently neural networks, have become standard to solve inverse problems over the last years. However, the theoretical recovery guarantees of such methods are still scarce and difficult to achieve. Only recently did unsupervised methods such as Deep Image Prior (DIP) get equipped with convergence and recovery guarantees for generic loss functions when trained through gradient flow with an appropriate initialization. In this paper, we extend these results by proving that these guarantees hold true when using gradient descent with an appropriately chosen step-size/learning rate. We also show that the discretization only affects the overparametrization bound for a two-layer DIP network by a constant and thus that the different guarantees found for the gradient flow will hold for gradient descent.

==> tex/sec_DIP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Case of The Two-Layer DIP Network}\label{sec:dip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{mdframed}[frametitle={Assumptions on the network input and intialization}]
%\begin{assumption}\label{ass:surjective_op}
%$\fop$ is a surjective linear operator; \vspace*{-.75em}
%\end{assumption}
\begin{assumption}\label{ass:u_sphere}
$\uv$ is a uniform vector on $\sph^{d-1}$;% \vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:w_init}
$\Wv(0)$ has iid entries from $\stddistrib$ and $\Cphi, \Cphid < +\infty$; %\vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:v_init}
$\Vv(0)$ is independent from $\Wv(0)$ and $\uv$ and has iid columns with identity covariance and $D$-bounded centered entries.%\vspace*{-.75em}
\end{assumption}
% \begin{assumption}\label{ass:phi_diff}
% $\phi$ is a twice differentiable function with $B$-bounded derivatives.
% \end{assumption}
% \begin{assumption}\label{ass:phi_lip}
% Both $\phi$ and $\phi'$ are $B$-Lipschitz, for some $B > 0$.
% \end{assumption}
\end{mdframed}



This section is devoted to studying under which conditions on the neural network architecture the key condition in \eqref{eq:bndR} is fulfilled. Towards this goal, we consider the case of a two-layer DIP network. Therein, $\uv$ is randomly set and kept fixed during the training, and the network is trained to transform this input into a signal that matches the observation $\yv$. In particular, we will provide bounds on the level of overparametrization ensuring that \eqref{eq:bndR} holds, which in turn will provide the subsequent recovery guarantees in Theorem~\ref{thm:main}. 

\subsection{The Two-Layer Neural Network}
We take $L=2$ in Definition~\ref{def:nn} and thus consider the network defined in~\eqref{eq:dipntk}:
\begin{align*}
    \gdip = \frac{1}{\sqrt{k}}\Vv\phi(\Wv\uv)
\end{align*}
with  $\Vv \in \R^{n \times k}$ and $\Wv \in \R^{k \times d}$, and $\phi$ an element-wise nonlinear activation function. Observe that it is immediate to account for the bias vector in the hidden layer by considering the bias as a column of the weight matrices $\Wv$, augmenting $\uv$ by 1 and then normalizing to unit norm. The normalization is required to comply with~\ref{ass:u_sphere} hereafter. The role of the scaling by $\sqrt{k}$ will become apparent shortly, but it will be instrumental to concentrate the kernel stemming from the jacobian of the network. 

% \todo[inline]{We do not have to impose these restrictions. I changed everything to handle the general case.}
% In the following analysis we use the mean-square error loss function to obtain exponential decay w.r.t time but other loss functions could be used resulting in other decays. Furthermore, we assume that $\fopnl$ is linear since it is the main use case of DIP~\cite{ulyanov_deep_2020} and we name it $\fop\in\R^{m\times n}$. 

In the sequel, we set $\Cphi = \sqrt{\Expect{X\sim\stddistrib}{\phi(X)^2}}$ and $\Cphid = \sqrt{\Expect{X\sim\stddistrib}{\phi'(X)^2}}$. We will assume without loss of generality that $\fopnl(0)=0$. This is a very mild assumption that is natural in the context of inverse problems, but can be easily removed if needed. We will also need the following assumptions:
\begin{mdframed}[frametitle={Assumptions on the network input and intialization}]
%\begin{assumption}\label{ass:surjective_op}
%$\fop$ is a surjective linear operator; \vspace*{-.75em}
%\end{assumption}
\begin{assumption}\label{ass:u_sphere}
$\uv$ is a uniform vector on $\sph^{d-1}$;% \vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:w_init}
$\Wv(0)$ has iid entries from $\stddistrib$ and $\Cphi, \Cphid < +\infty$; %\vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:v_init}
$\Vv(0)$ is independent from $\Wv(0)$ and $\uv$ and has iid columns with identity covariance and $D$-bounded centered entries.%\vspace*{-.75em}
\end{assumption}
% \begin{assumption}\label{ass:phi_diff}
% $\phi$ is a twice differentiable function with $B$-bounded derivatives.
% \end{assumption}
% \begin{assumption}\label{ass:phi_lip}
% Both $\phi$ and $\phi'$ are $B$-Lipschitz, for some $B > 0$.
% \end{assumption}
\end{mdframed}
%These assumptions are standard. Assumptions~\ref{ass:u_sphere}, \ref{ass:w_init} and \ref{ass:v_init} are quite common. Assumptions~\ref{ass:phi_diff} is met by many activations such as the softmax, sigmoid or hyperbolic tangent. Including the ReLU requires more technicalities that will be avoided here. 

\subsection{Recovery Guarantees in the Overparametrized Regime}
%
% Introduction où on présente le réseau avec la formule et tout
% Les hypothèses sur le réseau
% Théorème principal
% Preuves et lemme technique.
Our main result gives a bound on the level of overparameterization which is sufficient for \eqref{eq:bndR} to hold. 

\begin{theorem}\label{th:dip_two_layers_converge}
Suppose that assumptions \ref{ass:l_smooth}, \ref{ass:min_l_zero}, \ref{ass:phi_diff} and \ref{ass:F_diff} hold. Let $C$, $C'$ two positive constants that depend only on the activation function and $D$. Let:
\[
\LFz = \max_{\xv \in \Ball\pa{0,C\sqrt{n\log(d)}}} \norm{\Jf(\xv)}
\]
and
\[
\LLz = \max_{\vv \in \Ball\pa{0,C\LFz\sqrt{n\log(d)}+\sqrt{m}\pa{\norminf{\fopnl(\xvc)}+\norminf{\veps}}}} \frac{\norm{\nabla_\vv \lossy(\vv)}}{\norm{\vv-\yv}}.
\]
Consider the one-hidden layer network \eqref{eq:dipntk} where both layers are trained with the initialization satisfying \ref{ass:u_sphere} to \ref{ass:v_init} and the architecture parameters obeying
\begin{align*}
k \geq C' \sigminF^{-4} n \psi\pa{\frac{\LLz}{2}\pa{C\LFz \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}}}^2}^4 .
%k \geq C \kappa(\fop)^2n \pa{\sqrt{n}\pa{\sqrt{\log(d)} + 1} + \sqrt{m}}^2 .
%k \geq C_1 \kappa(\fop)^2 n^{5/2}m 
\end{align*}
Then \eqref{eq:bndR} holds with probability at least $1 - 2n^{-1} - d^{-1}$.
%will converge exponentially fast to the optimal solution in measurement space up to the noise level such that
%\begin{align*}
%    \frac{\norm{\yzy}}{\sigminA} < \frac{\sigminjgz^2}{2\Lip(\jcal)}
%\end{align*}
% \begin{align*}
% \norm{\yvt - \yvc} \leq 2 \norm{\veps} \qquad \text{for all} \qquad t \geq \frac{C_2m\log\left(\norm{\yv - \fop \mathbf{g}(\uv,\Wv(0))}\right)}{\sigminA^2\Cphid^2} 
% \end{align*}
% \begin{align}
%     \norm{\yvt - \yv}^2 \leq  \norm{\yvz - \yv}^2 \exp\left\{-\frac{1}{4}\sigmin\left(\fop\jthetaz\right) t\right\},
% \end{align}
%with probability at least $1 - n^{-1} - d^{-1} - \exp(-n)$, where $C_i$ are positive constants that depend only on the activation function and the bound $D$.
\end{theorem}

% Discussion
Before proving Theorem~\ref{th:dip_two_layers_converge}, a few remarks are in order. 


\begin{remark}[Randomness of $\Sigma'$]
It is worth observing that since the initialization is random, so is the set of signals $\Sigma'=\Sigma_{\Ball_{R'+\norm{\thetavz}}(0)}$ by definition, where $\thetavz=(\Vv(0),\Wv(0))$. This set is contained in a larger  deterministic set with high probability. Indeed, Gaussian concentration gives us, for any $\delta > 0$,
\[
\normf{\Wv(0)} \leq (1+\delta)\sqrt{kd}
\]
with probability larger than $1-e^{-\delta^2 kd/2}$. Moreover, since by \ref{ass:v_init} $\Vv(0)$ has independent columns with bounded entries and $\Expect{}{\norm{\Vv_i(0)}^2}=n$, we can apply Hoeffding's inequality to $\normf{\Vv(0)}^2=\sum_{i=1}^k\norm{\Vv_i(0)}^2$ to infer that
\[
\normf{\Vv(0)} \leq (1+\delta)\sqrt{kn}
\]
with probability at least $1-e^{-\delta^2 kd/(2D^2)}$. Collecting the above, we have
\[
\norm{\thetavz} \leq (1+\delta)\sqrt{k}\pa{\sqrt{n}+\sqrt{d}} ,
\]
with probability at least $1-e^{-\delta^2 kd/2}-e^{-\delta^2 kd/(2D^2)}$. In view of the bound on $R'$ (see \eqref{eq:R'Rbnd}), this yields that with probability at least $1-e^{-\delta^2 kd/2}-e^{-\delta^2 kd/(2D^2)}-2n^{-1}-d^{-1}$, $\Sigma' \subset \Sigma_{\Ball_{\rho}(0)}$, where
{\small{
\[
\rho = \frac{4}{\sigminF\sqrt{\Cphi^2 + \Cphid^2}}\psi\pa{\frac{\LLz}{2}\pa{C\LFz \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}}}^2} + (1+\delta)\sqrt{k}\pa{\sqrt{n}+\sqrt{d}} .
\]
}}
This confirms the expected behaviour that expressivity of $\Sigma'$ is higher as the overparametrization increases.
\end{remark}


\begin{remark}[Distribution of $\uv$]
The generator $\gv(\cdot,\thetav)$ synthesize data by transforming the input (latent) random variable $\uv$. As such, it generates signals $\xv \in \Sigma'$ who are in the support of the measure $\gv(\cdot,\thetav) \# \mu_{\uv}$, where $\mu_{\uv}$ is the distribution of $\uv$, and $\#$ is the push-forward operator. Expressivity of these generative models, coined also push-forward models, in particular GANs, have been recently studied either empirically or theoretically \cite{Khayatkhoei,Gurumurthy,Tanielian,Salmona,Issenhuth}. In particular, this literature highlights the known fact that, since $\gv(\cdot,\thetav)$ is continuous by construction, the support of $\gv(\cdot,\thetav) \# \mu_{\uv}$ is connected if that of $\mu_{\uv}$ is connected (as in our case). On the other hand, a common assumption in the imaging literature, validated empirically by \cite{Pope}, is that distributions of natural images are supported on low dimensional manifolds. It is also conjectured that the distribution of natural images may in fact lie on a union of disjoint manifolds rather than one globally connected manifold; the union of subspaces or manifolds model is indeed a common assumption in signal/image processing. In the latter case, a generator $\gv(\cdot,\thetav)$ that will attempt to cover the different modes (manifolds) of the target distribution from one unimodal latent variable $\uv$ will generate samples out of the real data manifold. There are two main ways to avoid this: either making the support of $\mu_{\uv}$ disconnected (e.g. using a mixture of distributions \cite{Gurumurthy,Hagemann}), or making $\gv(\cdot,\thetav)$ discontinuous \cite{Khayatkhoei}. The former strategy appears natural in our context and it will be interesting to investigate this generalization in a future work.
\end{remark}


\begin{remark}[Restricted injectivity]
As argued above, if $\Sigma'$ belongs to a target manifold $\cM$, then the restricted injectivity condition \eqref{ass:lin_inj} tells us that $\fop$ has to be invertible on the tangent cone of the target manifold $\cM$ at the closest point of $\xvc$ in $\cM$. 
\end{remark}


\begin{remark}[Dependence on $\LLz$ and $\LFz$]
The overparametrization bound on $k$ depends on $\LLz$ and $\LFz$ which in turn may depend on $(n,m,d)$. Their estimate is therefore important. For instance, if $\fopnl$ is globally Lipschitz, as is the case when it is linear, then $\LFz$ is independent of $(n,m,d)$. As far as $\LLz$ is concerned, it is of course independent of $(n,m,d)$ if the loss gradient is globally Lipschitz continuous. Another situation of interest is when $\nabla_{\vv}\lossy(\vv)$ verifies
\[
\norm{\nabla_\vv\lossy(\vv) - \nabla_\zv\lossy(\zv)} \leq \varphi\pa{\norm{\vv-\zv}}, \quad \forall \vv,\zv \in \R^m ,
\]
where $\varphi: \R_+ \to \R_+$ is increasing and vanishes at $0$.
This is clearly weaker than global Lipschitz continuity and covers it as a special case. It also encompasses many important situations such as e.g. losses with H\"olderian gradients. It then easily follows, see e.g. \cite[Theorem~18.13]{BauschkeBook}, that for all $\vv \in \R^m$:
\[
\lossy(\vv) \leq \Phi\pa{\norm{\vv-\yv}} \qwhereq \Phi(s) = \int_0^1 \frac{\varphi(st)}{t} \dt .
\]
In this situation, and if $\fopnl$ is also globally $\LF$-Lipschitz, following our line of proof, the overparametrization bound of Theorem~\ref{th:dip_two_layers_converge} reads
\begin{align*}
k \geq C' \sigminF^{-4} n \psi\pa{\Phi\pa{C\LF \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}}}}^4 .
\end{align*}
\end{remark}

%\todo[inline]{Rewrite the following two remarks. First comment on the scaling in the general case and that in particular depend on the desingularizing function $\psi$. Then specialize to the case of a linear forward operator.}

\begin{remark}[Dependence on the loss function]
    If we now take interest in the scaling of the overparametrization bound on $k$ with respect to $(n,m,d)$ in the general case we obtain that $k\gtrsim \sigminF^{-4} n \psi(\LLz(\LFz^2 n + m))^4$. Aside from the possible dependence of $\LLz$ and $\LFz$ on the parameters $(n,m,d)$ discussed before, we observe that this bound is highly dependent on the desingularizing function $\psi$ given by the loss function. In the \L ojasiewicz case where $\psi = cs^\alpha$ with $\alpha \in [0,1]$, one can choose to use a sufficiently small $\alpha$ to reduce the scaling on the parameters but then one would slow the convergence rate as described in Corollary~\ref{col:loja_rate} which implies a tradeoff between the convergence rate and the number of parameters to ensure this convergence.
    
    In the special case where $\alpha = \frac{1}{2}$ which corresponds to the MSE loss, and where  $\LFz$ is of constant order and independent of $(n,m,d)$, then the overperametrization of $k$ necessary for ensuring convergence to a zero-loss is $k\gtrsim n^3m^2$. Another interesting case is when $\fopnl$ is linear. In that setting, the overparametrization bound becomes $k\gtrsim \sigminF^{-4} n \psi(\LLz(\norm{\fopnl}^2 n + m))^4$. By choosing the MSE loss, and thus controlling $\psi$ to be a square root operator, then we obtain that we need $k\gtrsim \kappa(\fopnl)^4 n^3m^2$. The bound is thus more demanding as $\fopnl$ becomes more and more ill-conditioned. The latter dependency can be interpreted as follows: the more ill-conditioned the original problem is, the larger the network needs to be. 
\end{remark}
\begin{remark}[Scaling when $\Vv$ is fixed]\label{rq:V_fixed}
    When the linear layer $\Vv$ is fixed and only $\Wv$ is trained, the overparametrization bound to guarantee convergence can be improved (see Appendix~\ref{appendix:V_fixed} and the results in~\cite{buskulic2023convergence}). In this case, one needs $k\gtrsim \sigminF^{-2} n \psi(\LLz(\LFz^2 n + m))^2$. In particular, for the MSE loss and an operator such that $\LFz$ is of constant order (as is the case when $\fopnl$ is linear), we only need $k \gtrsim n^{2}m$. The main reason underlying this improvement is that there is no need in this case to control the deviation of $\Vv$ from its initial point to compute the local Lipschitz constant of the jacobian of the network. This allows to have a far better Lipschitz constant estimate which turns out to be even global in this case.
\end{remark}
\begin{remark}[Effect of input dimension $d$]
    Finally, the dependence on $d$ is far smaller (by a log factor) than the one on $n$ and $m$. In the way we presented the theorem, it does also affect the probability obtained but it is possible to write the same probability without $d$ and with a stronger impact of $n$. This indicates that $d$ plays a very minor role on the overparametrization level whereas $k$ is the key to reaching the overparametrized regime we are looking for. In fact, this is demonstrated by our numerical experiments where we obtained the same results by using very small $d \in [1,10]$ or larger values up to 500, for all our experiments with potentially large $n$.
\end{remark}

% \begin{remark}
% We start with the scaling of the network architecture parameters required. First, the bound on $k$, the number of neurons of the hidden layer, scales quadratically in $n^2$ and linearly in $m$. We thus have the bound $k \gtrsim n^2m$. The probability of success in our theorem is also dependent on the architecture parameters. More precisely, this probability increases with growing number of observations.
% \end{remark}
% %the probability with which our result holds grows with the problem size. The only part in this probability depending on the problem size is the ratio $km/(\sqrt{k} + \sqrt{n})^2$ in the third term. Since $k$ is of the order $n^2m$, it means that this ratio will be of the order $m$ which means that the probability will increase with the problem size as desired. \textbf{cinq dernieres lignes pas hyper clair !}

% % Discuss proba of d
% \begin{remark}
% The other scaling of the theorem is on the input size $d$ and informs us that $d$ and its influence is logarithmic. The bound is more demanding as $\fop$ becomes more ill-conditioned. The latter dependency can be interpreted as follows: the more ill-conditioned the original problem is, the larger the network needs to be. Let us emphasize that, contrary to other learning settings in the literature, the size $d$ of the random input  $\uv$ is free, and so far it has remained unclear how to choose it. Our result provides an first  answer for shallow networks in the overparametrized setting: most of the overparametrization necessary for the optimization to converge is due to $k$.
% \end{remark}

%On our way to prove \eqref{thm:main}, we actually show that $\yv(t)$ converges exponentially to $\yv$, which is converted to a recovery of $\yvc$ through an early stopping strategy. This ensures that the network does not overfit the noise and provides a solution in a ball around $\yvc$ whose radius is linear in the noise level (so-called prediction linear convergence in the inverse problem literature). This provides a first result on convergence of wide DIP networks that ensures they behave well in the observation space. One has to keep in mind, however, that this does not say anything about the recovered vector generated by the network and its relation to $\xvc$ (in absence of noise and at convergence, it might be any element of $\xvc + \text{ker}(\fop)$). This is a much more challenging question that we leave to a future work.

%Furthermore, the theorem informs us that once the overparametrization bounds are respected, the network can achieve a perfect match in the observation space between its transformed output and its target observation with an exponential convergence rate. This shows that under the right condition, Deep Inverse Priors models, even with a shallow network, are able to find a signal that will correspond in the measurement space to the target which is the task they are trained for. Of course, it is important to remember that this means that the network will overfit the noise and thus, we are confident that the signal will be matched up to an error depending on the norm of the noise.

\subsection{Proofs}
We start with the following lemmas that will be instrumental in the proof of Theorem~\ref{th:dip_two_layers_converge}.

\begin{lemma}[Bound on $\sigminjgz$ with both layers trained]
\label{lemma:min_eigenvalue_singvalue_init_both_layer}
Consider the one-hidden layer network \eqref{eq:dipntk} with both layers trained under assumptions \ref{ass:phi_diff} and \ref{ass:u_sphere}-\ref{ass:v_init}. We have
\begin{align*}
\sigminjgz \geq \sqrt{\Cphi^2 + \Cphid^2}/2 
\end{align*}
%with probability $1 - 2 \exp{(-c\tau^2)}$. Here, $C$, $c > 0$ depend only on the sub-gaussian norm $\normsubgauss{\phidW_1 \Vv_1}$ 
with probability at least $1-2n^{-1}$ provided that $k/\log(k) \geq C n\log(n)$ for $C > 0$ large enough that depends only on $B$, $\Cphi$, $\Cphid$ and $D$.
\end{lemma}

\begin{proof}

Define the matrix $\Hv = \jthetaz\jthetaz\tp$. Since $\uv$ is on the unit sphere, $\Hv$ reads
\begin{align*}
    \Hv = \frac{1}{k} \sum_{i=1}^k \Hv_i, \qwhereq \Hv_i \eqdef \phi'(\Wv^i(0)\uv)^2\Vv_i(0)\Vv_i(0)\tp + \phi(\Wv^i(0)\uv)^2\Id_n .
\end{align*}
It then follows that
\begin{align*}
    \Expect{}{\Hv} &= \frac{1}{k}\Expect{X\sim \stddistrib}{\phi'(X)^2} \sum_{i=1}^k\Expect{}{\Vv_i(0) \Vv_i(0)\tp} + \Expect{X\sim \stddistrib}{\phi(X)^2}\Id_n\\
    &= (\Cphid^2 + \Cphi^2) \Id_n,
\end{align*}
where we used \ref{ass:u_sphere}, \ref{ass:w_init} and orthogonal invariance of the Gaussian distribution, hence $\Wv^i(0)\uv$ are iid in $\stddistrib$, as well as \ref{ass:v_init} and independence between $\Vv(0)$ and $\Wv(0)$. Moreover, $\Expect{}{\phi(X)} \leq \Cphi$, and since $X\sim\stddistrib$ and in view of \ref{ass:phi_diff}, we can upper-bound $\phi(X)$ using the Gaussian concentration inequality to get
\begin{align}
    \prob{\phi(X) \geq \Cphi\sqrt{\log(nk)} + \tau} \leq \prob{\phi(X) \geq \Expect{}{\phi(X)} + \tau}
    \leq \exp{\left(-\frac{\tau^2}{2B^2}\right)}.
\end{align}
By choosing $\tau = \sqrt{2}B\sqrt{\log(nk)}$, and taking $c_1 = \Cphi + \sqrt{2}B$, we get
\begin{align}
    \prob{\phi(X) \geq c_1\sqrt{\log(nk)}} \leq (nk)^{-1} .
\end{align}
Using a union bound, we obtain
\begin{align*}
\prob{\max_{i \in [k]} \phi(\Wv^i(0)\uv)^2 > c_1\log(nk)} \leq n(nk)^{-1} \leq n^{-1} .
    %&\tau^2 \geq 2B^2n\log(k)C_1^2 \qquad \text{and}\\
    %&\Expect{}{\phi(X)} + \tau \leq \sqrt{2} B C_2\sqrt{n\log(k)},
\end{align*}
% with $C_1, C_2 > 0$ depending on $\phi$. We now apply the concentration inequality and together with an union bound, we get that with probability $1-\exp(-n)$, $\forall i \in \{1,...,k\}$
% \begin{align*}
%     \phi(\Wv^i\uv)^2 \leq 2B^2C_2^2n\log(k).
% \end{align*}
Thus, with probability at least $1-n^{-1}$ we get
\begin{align*}
\max_{i \in [k]} \lmax\pa{\Hv_i} 
\leq B^2D^2n + c_1\log(nk)
\leq c_2n\log(k) , % B^2nC_3\log(k).
\end{align*}
where $c_2 = B^2D^2 + 2c_1$.
We can then apply the matrix Chernoff inequality \cite[Theorem~5.1.1]{tropp_introduction_2015} to get
% \[
% \prob{\sigminjgz \leq \delta\sqrt{\Cphid^2 + \Cphi^2}} \leq ne^{-\frac{(1-\delta)^2k(\Cphid^2 + \Cphi^2)}{2B^2C_3n\log(k)}} .
% \]
\begin{align*}
&\prob{\sigminjgz \leq \delta\sqrt{\Cphid^2 + \Cphi^2}} \\
&\leq \prob{\sigminjgz \leq \delta\sqrt{\Cphid^2 + \Cphi^2} \; \bigg| \max_{i \in [k]} \lmax\pa{\Hv_i} \leq c_2n\log(k)}
+ \prob{\max_{i \in [k]} \lmax\pa{\Hv_i} \geq c_2n\log(k)} \\
&\leq ne^{-\frac{(1-\delta)^2k(\Cphid^2 + \Cphi^2)}{c_2n\log(k)}} + n^{-1} .
\end{align*}
Taking $\delta=1/2$ and $k$ as prescribed with a sufficiently large constant $C$, we conclude.

\end{proof}

% lemma Lipschitz constant

%\todo[inline]{The following lemma was completely incorrect. $\jcal$ is only locally Lipschitz continuous but not globally so (it is only globally Lipschitz continuous for the fixed $\Vv$). I corrected the statement and the proof accordingly. I is worth also stating another result when training only $\Wv$ as the scaling is much better.}

\begin{lemma}[Local Lipschitz constant of $\jcal$ with both layers trained]\label{lemma:lip-Jacobian-both-layers}
Suppose that assumptions \ref{ass:phi_diff}, \ref{ass:u_sphere} and \ref{ass:v_init} are satisfied. For the one-hidden layer network \eqref{eq:dipntk} with both layers trained, we have for $n \geq 2$ and any $\rho > 0$:
\[
\Lip_{\Ball(\thetavz,\rho)}(\jcal) \leq B (1+2(D+\rho))\sqrt{\frac{n}{k}} .
\]
\end{lemma}

\begin{proof}
Let $\thetav \in \R^{k(d + n)}$ (resp. $\thetavalt$) be the vectorized form of the parameters of the network $(\Wv,\Vv)$ (resp. $(\Wvalt,\Vvalt)$). For $\thetav, \thetavalt \in \Ball(R,\thetavz)$, we have
 
\begin{align*}
\norm{\jtheta - \jcal(\thetavalt)}^2
%&\leq \frac{1}{k} \left(\normf{\sum_{i=1}^k (\phi'(\Wv^i\uv)\Vv_i - \phi'(\Wvalt^i\uv)\Vvalt_i)\uv\tp}^2 + \normf{\sum_{i=1}^k (\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)) \Id_n}^2\right)\\
&\leq \frac{1}{k} \pa{\sum_{i=1}^k \normf{\phi'(\Wv^i\uv)\Vv_i\uv\tp - \phi'(\Wvalt^i\uv)\Vvalt_i\uv\tp}^2 + \normf{\ddiag{n}{\phiWu - \phiWualt}}^2}\\
&\leq \frac{1}{k} \Bigg(2 \sum_{i=1}^k \pa{\normf{\phi'(\Wv^i\uv)\pa{\Vv_i - \Vvalt_i}\uv\tp}^2 + \normf{\pa{\phi'(\Wv^i\uv)-\phi'(\Wvalt^i\uv)}\Vvalt_i\uv\tp}^2} \\
&\qquad + \normf{\ddiag{n}{\phiWu - \phiWualt}}^2\Bigg)\\
&\leq \frac{1}{k} \pa{2 B^2 \sum_{i=1}^k \pa{\norm{\Vv_i - \Vvalt_i}^2 + \norm{\Wv^i-\Wvalt^i}^2\norm{\Vvalt_i}^2} + n\norm{\phiWu - \phiWualt}^2}\\
&\leq \frac{1}{k} \pa{2 B^2 \normf{\Vv - \Vvalt}^2 + 2B^2\sum_{i=1}^k\norm{\Wv^i-\Wvalt^i}^2\norm{\Vvalt_i}^2 +  B^2n\norm{(\Wv - \Wvalt)\uv}^2}\\
&\leq \frac{1}{k} \pa{2 B^2 \normf{\Vv - \Vvalt}^2 + 2B^2\max_i\norm{\Vvalt_i}^2\normf{\Wv-\Wvalt}^2 +  B^2n\normf{\Wv - \Wvalt}^2}\\
%&= \frac{1}{k} \left(\norm{\sum_{i=1}^k (\phi'(\Wv^i\uv)\Vv_i - \phi'(\Wvalt^i\uv)\Vvalt_i)}^2 + \normf{\sum_{i=1}^k (\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)) \Id_n}^2\right)\\
%&= \frac{1}{k} \left(\norm{\sum_{i=1}^k (\phi'(\Wv^i\uv)\Vv_i - \phi'(\Wvalt^i\uv)\Vvalt_i)}^2 + n\norm{\phiWu - \phiWualt}^2\right)\\
%&\leq  \frac{1}{k} \left(B^2\sum_{i=1}^k\norm{\Vv_i - \Vvalt_i}^2 + \normf{\sum_{i=1}^k (\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)) \Id_n}^2\right)\\
%&\leq  \frac{1}{k} \left(B^2\sum_{i=1}^k\norm{\Vv_i - \Vvalt_i}^2 + B^2n\norm{\Wv\uv - \Wvalt\uv}^2\right)\\
&\leq  \frac{n}{k}B^2\pa{\normf{\Vv - \Vvalt}^2 + \normf{\Wv - \Wvalt}^2} + \frac{2}{k}B^2\max_i\norm{\Vvalt_i}^2\normf{\Wv-\Wvalt}^2\\
% &\leq  \frac{1}{k} \left(B^2\normf{\Vv - \Vvalt}^2 + \normf{\sum_{i=1}^k (\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)) \Id_n}^2\right)\\
% &\leq  \frac{1}{k} \left(B^2\normf{\Vv - \Vvalt}^2 + n\sum_{i=1}^k |\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)|^2\right)\\
% &\leq  \frac{1}{k} B^2 \left(\normf{\Vv - \Vvalt}^2 + n\sum_{i=1}^k \norm{\Wv^i\uv - \Wvalt^i\uv}^2\right)\\
% &\leq  \frac{n}{k} B^2 \left(\normf{\Vv - \Vvalt}^2 + \normf{\Wv - \Wvalt}^2\right)\\
&=  \frac{n}{k} B^2 \norm{\thetav - \thetavalt}^2 + \frac{2}{k}B^2\max_i\norm{\Vvalt_i}^2\normf{\Wv-\Wvalt}^2 .
\end{align*}
Moreover, for any $i \in [k]$:
\[
\norm{\Vvalt_i}^2 \leq 2\norm{\Vv_i(0)}^2 + 2 \norm{\Vvalt_i-\Vv_i(0)}^2 \leq 2\norm{\Vv_i(0)}^2 + 2 \norm{\thetav-\thetavz}^2 \leq 2nD^2 + 2\rho^2 ,
\]
where we used \ref{ass:v_init}.
Thus
\begin{align*}
\norm{\jtheta - \jcal(\thetavalt)}^2 \leq \frac{n}{k} B^2\pa{1+4D^2+2\rho^2}\norm{\thetav - \thetavalt}^2 .
\end{align*}
\end{proof}

% \begin{lemma}[Bound on the initial error]\label{lemma:bound_initial_misfit}
% Under the main assumptions, the initial error of the network is bounded by
% \begin{align*}
% \norm{\yv(0) - \yv} \leq \norm{\fop}\pa{C \sqrt{n\log(d)} + \sqrt{n}\norminf{\xvz} + \sqrt{m}\norminf{\veps}},
% \end{align*}
% with probability at least $1 - d^{-1}$.
% \end{lemma}

% \begin{proof}
% We first observe that
% \[
% \norm{\yvz - \yv} \leq \norm{\fop}\norm{\gdipz} + \norm{\fop}\pa{\sqrt{n} \norminf{\xvc} + \sqrt{m} \norminf{\veps}} ,
% \]
% where $\gdipz = \frac{1}{\sqrt{k}} \sum_{i=1}^k \phi(\Wv^i\uv)\Vv_i$. We now prove that this term concentrates around its expectation. First, we have by independence
% \[
% \Expect{}{\norm{\gdipz}}^2 \leq \frac{1}{k}\Expect{}{\norm{\sum_{i=1}^k \phi(\Wv^i\uv)\Vv_i}^2} = \Expect{}{\phi(\Wv^1\uv)^2\norm{\Vv_1}^2} = \Cphi^2 n .
% \]
% In addition,
% \begin{align*}
% &\abs{\norm{\mathbf{g}(\uv,\Wv)} - \norm{\mathbf{g}(\uv,\Wvalt)}} 
% \leq \frac{1}{\sqrt{k}}\norm{\sum_{i=1}^k \pa{\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)}\Vv_i} \\
% &\leq BD\sqrt{n}\pa{\frac{1}{\sqrt{k}}\sum_{i=1}^k \norm{\Wv^i - \Wvalt^i}} \leq BD\sqrt{n}\normf{\Wv - \Wvalt} .
% \end{align*}
% We then get
% \begin{align*}
% &\prob{\norm{\mathbf{g}(\uv,\Wv(0))} \geq \Cphi \sqrt{n\log(d)} + \tau} \\
% &\leq \prob{\norm{\mathbf{g}(\uv,\Wv(0))} \geq \Expect{}{\norm{\gdipz}} + \tau}\\ 
% &\leq e^{-\frac{\tau^2}{2\Lip(\norm{\mathbf{g}(\uv,\Wv(0))})^2}} \leq e^{-\frac{\tau^2}{2nB^2D^2}} .
% \end{align*}
% Taking $\tau = \sqrt{2}BD \sqrt{n\log(d)}$, we get the desired claim. 
% \end{proof}

\begin{lemma}[Bound on the initial error]\label{lemma:bound_initial_misfit}
Under assumptions \ref{ass:phi_diff}, \ref{ass:F_diff} and \ref{ass:u_sphere} to \ref{ass:v_init}, the initial error of the network satisfies
\begin{align*}
\norm{\yv(0) - \yv} \leq C\LFz \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}} ,
\end{align*}
with probability at least $1 - d^{-1}$, where $C$ is a constant that depends only on $B$, $\Cphi$, and $D$.
\end{lemma}

\begin{proof}
By \ref{ass:F_diff} and the mean value theorem, we have
\[
\norm{\yvz - \yv} \leq \max_{\xv \in \Ball(0,\norm{\xvz})} \norm{\Jf(\xv)}\norm{\xvz} + \sqrt{m} \pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}} ,
\]
where $\xvz = \gdipz = \frac{1}{\sqrt{k}} \sum_{i=1}^k \phi(\Wv^i(0)\uv)\Vv_i(0)$. Moreover, by \ref{ass:v_init}:
\[
\norm{\gdipz} \leq \max_i \norm{\Vv_i(0)} \frac{1}{\sqrt{k}} \sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)} \leq D\sqrt{n} \frac{1}{\sqrt{k}} \sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)} .
\]

We now prove that the last term concentrates around its expectation. First, owing to \ref{ass:u_sphere} and \ref{ass:w_init}, we can argue using orthogonal invariance of the Gaussian distribution and independence to infer that
\[
\Expect{}{\frac{1}{\sqrt{k}} \sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)}}^2 \leq \frac{1}{k}\Expect{}{\pa{\sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)}}^2} = \Expect{}{\phi(\Wv^1(0)\uv)^2} = \Cphi^2 .
\]
In addition, the triangle inequality and Lipschitz continuity of $\phi$ (see \ref{ass:phi_diff}) yields
\begin{align*}
\frac{1}{\sqrt{k}}\abs{\sum_{i=1}^k \abs{\phi(\Wv^i\uv)} - \abs{\phi(\Wvalt^i\uv)}}
&\leq \frac{1}{\sqrt{k}}\sum_{i=1}^k \abs{\phi(\Wv^i\uv) - \phi(\Wvalt^i\uv)} \\
&\leq B\pa{\frac{1}{\sqrt{k}}\sum_{i=1}^k \norm{\Wv^i - \Wvalt^i}} \leq BD\normf{\Wv - \Wvalt} .
\end{align*}
We then get using the Gaussian concentration inequality that
\begin{align*}
&\prob{\frac{1}{\sqrt{k}} \sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)} \geq \Cphi \sqrt{\log(d)} + \tau} \\
&\leq \prob{\frac{1}{\sqrt{k}} \sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)} \geq \Expect{}{\frac{1}{\sqrt{k}} \sum_{i=1}^k \abs{\phi(\Wv^i(0)\uv)}} + \tau}
\leq e^{-\frac{\tau^2}{2B^2D^2}} .
\end{align*}
Taking $\tau = \sqrt{2}BD \sqrt{\log(d)}$, we get
\[
\norm{\xvz} \leq C \sqrt{n\log(d)} 
\] 
with probability at least $1-d^{-1}$. Since the event above implies $\Ball(0,\norm{\xvz}) \subset \Ball\pa{0,C\sqrt{n\log(d)}}$, we conclude.
\end{proof}


\begin{proof}[Proof of Theorem~\ref{th:dip_two_layers_converge}]
Proving Theorem~\ref{th:dip_two_layers_converge} amounts to showing that \eqref{eq:bndR} holds with high probability under our scaling. This will be achieved by combining Lemma~\ref{lemma:min_eigenvalue_singvalue_init_both_layer}, Lemma~\ref{lemma:lip-Jacobian-both-layers} and Lemma~\ref{lemma:bound_initial_misfit} as well as the union bound.

From Lemma~\ref{lemma:min_eigenvalue_singvalue_init_both_layer}, we have
\begin{align*}
\sigminjgz \geq \sqrt{\Cphi^2 + \Cphid^2}/2 
\end{align*}
with probability at least $1-2n^{-1}$ provided $k \geq C_0 n\log(n)\log(k)$ for $C_0 > 0$. On the other hand, from Lemma~\ref{lemma:lip-Jacobian-both-layers}, and recalling $R$ from \eqref{eq:RandR'}, we have that $R$ must obey
\[
R \geq \frac{\sigminjgz}{2B((1+2D)+2R))}\sqrt{\frac{k}{n}} \geq \frac{\sqrt{\Cphi^2 + \Cphid^2}}{8B((1/2+D)+R))}\sqrt{\frac{k}{n}} .
\]
Solving for $R$, we arrive at
\[
R \geq \frac{\sqrt{(1/2+D)^2 + \frac{\sqrt{(\Cphi^2 + \Cphid^2)\frac{k}{n}}}{2B}}-(1/2+D)}{2}.
\]
Simple algebraic computations and standard bounds on $\sqrt{1+a}$ for $a \in [0,1]$ show that
\[
R \geq C_1\pa{\frac{k}{n}}^{1/4}
\]
whenever $k \gtrsim n$, $C_1$ being a positive constant that depends only on $B$, $\Cphi$, $\Cphid$ and $D$.

Thanks to \ref{ass:l_smooth} and \ref{ass:min_l_zero}, we have by the descent lemma, see e.g. \cite[Lemma~2.64]{BauschkeBook}, that
\[
\lossyzy \leq \max_{\vv \in [\yv,\yvz]}\frac{\norm{\nabla \lossy(\vv)}}{\norm{\vv-\yv}} \frac{\norm{\yvz-\yv}^2}{2} .
\] 
Combining Lemma~\ref{lemma:bound_initial_misfit} and the fact that 
\[
[\yv,\yvz] \subset \Ball(0,\norm{\yv}+\norm{\yvz}) 
\]
then allows to deduce that with probability at least $1-d^{-1}$, we have
\[
\lossyzy \leq \frac{\LLz}{2}\pa{C\LFz \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}}}^2 .
\] 
Therefore, using the union bound and the fact that $\psi$ is increasing, it is sufficient for \eqref{eq:bndR} to be fulfilled with probability at least $1-2n^{-1}-d^{-1}$, that
\begin{equation}\label{eq:R'Rbnd}
\frac{4}{\sigminF\sqrt{\Cphi^2 + \Cphid^2}}\psi\pa{\frac{\LLz}{2}\pa{C\LFz \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fopnl(\xvc)} + \norminf{\veps}}}^2} < C_1\pa{\frac{k}{n}}^{1/4} ,
\end{equation}
whence we deduce the claimed scaling.
\end{proof}




==> tex/sec_DIP_discr.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Case of The Two-Layer DIP Network}\label{sec:dip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this 

This section is devoted to studying under which conditions on the neural network architecture the key condition in \eqref{eq:bndR} is fulfilled. Towards this goal, we consider the case of a two-layer DIP network. Therein, $\uv$ is randomly set and kept fixed during the training, and the network is trained to transform this input into a signal that matches the observation $\yv$. In particular, we will provide bounds on the level of overparametrization ensuring that \eqref{eq:bndR} holds, which in turn will provide the subsequent recovery guarantees in Theorem~\ref{thm:main}. 

\subsection{The Two-Layer Neural Network}
We take $L=2$ in Definition~\ref{def:nn} and thus consider the network defined in~\eqref{eq:dipntk}:
\begin{align}\label{eq:dipntk}
    \gdip = \frac{1}{\sqrt{k}}\Vv\phi(\Wv\uv)
\end{align}
with  $\Vv \in \R^{n \times k}$ and $\Wv \in \R^{k \times d}$, and $\phi$ an element-wise nonlinear activation function. Observe that it is immediate to account for the bias vector in the hidden layer by considering the bias as a column of the weight matrices $\Wv$, augmenting $\uv$ by 1 and then normalizing to unit norm. The normalization is required to comply with~\ref{ass:u_sphere} hereafter. The role of the scaling by $\sqrt{k}$ will become apparent shortly, but it will be instrumental to concentrate the kernel stemming from the jacobian of the network. 

In the sequel, we set $\Cphi = \sqrt{\Expect{X\sim\stddistrib}{\phi(X)^2}}$ and $\Cphid = \sqrt{\Expect{X\sim\stddistrib}{\phi'(X)^2}}$. We will assume without loss of generality that $\fopnl(0)=0$. This is a very mild assumption that is natural in the context of inverse problems, but can be easily removed if needed. We will also need the following assumptions:

\begin{mdframed}[frametitle={Assumptions on the network input and intialization}]
%\begin{assumption}\label{ass:surjective_op}
%$\fop$ is a surjective linear operator; \vspace*{-.75em}
%\end{assumption}
\begin{assumption}\label{ass:u_sphere}
$\uv$ is a uniform vector on $\sph^{d-1}$;% \vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:w_init}
$\Wv(0)$ has iid entries from $\stddistrib$ and $\Cphi, \Cphid < +\infty$; %\vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:v_init}
$\Vv(0)$ is independent from $\Wv(0)$ and $\uv$ and has iid columns with identity covariance and $D$-bounded centered entries.%\vspace*{-.75em}
\end{assumption}
% \begin{assumption}\label{ass:phi_diff}
% $\phi$ is a twice differentiable function with $B$-bounded derivatives.
% \end{assumption}
% \begin{assumption}\label{ass:phi_lip}
% Both $\phi$ and $\phi'$ are $B$-Lipschitz, for some $B > 0$.
% \end{assumption}
\end{mdframed}

Our main result gives a bound on the level of overparameterization which is sufficient for \eqref{eq:bndR2} to hold. 

\begin{corollary}\label{cor:dip_two_layers_converge_discr}
Suppose that assumptions \ref{ass:l_smooth}, \ref{ass:min_l_zero} and \ref{ass:phi_diff} hold. Let $C$, $C'$ two positive constants that depend only on the activation function and $D$. Let:
\[
\LLz = \max_{\vv \in \Ball\pa{0,C\norm{\fop}\sqrt{n\log(d)}+\sqrt{m}\pa{\norminf{\fop\xvc}+\norminf{\veps}}}} \frac{\norm{\nabla_\vv \lossy(\vv)}}{\norm{\vv-\yv}}.
\]
Consider the one-hidden layer network \eqref{eq:dipntk} where both layers are trained with the initialization satisfying \ref{ass:u_sphere} to \ref{ass:v_init} and the architecture parameters obeying
\begin{align*}
k \geq C' \sigminA^{-4} n \psi\pa{\frac{\norm{\fop}}{2}\pa{C\LFz \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}}}^2}^4 .
%k \geq C \kappa(\fop)^2n \pa{\sqrt{n}\pa{\sqrt{\log(d)} + 1} + \sqrt{m}}^2 .
%k \geq C_1 \kappa(\fop)^2 n^{5/2}m 
\end{align*}
Then \eqref{eq:bndR2} holds with probability at least $1 - 2n^{-1} - d^{-1}$.
\end{corollary}

% Discussion théorème

\begin{proof}
    The only difference between the $R$ and $R'$ from~\eqref{eq:bndR2} and the ones from~\cite[Theorem~3.2]{buskulic2023convergenceJournal} is that $R'$ in our case is multiplied by a constant factor. This allows us to prove this corollary using the same proof structure as the one for~\cite[Theorem~4.1]{buskulic2023convergenceJournal} that we adapt to take the constant in $R'$ into account and the fact that our operator is linear.
    
    Due to the fact that the assumptions of the original Theorem and this corollary are the same, it means that both~\cite[Lemma~4.9]{buskulic2023convergenceJournal} and~\cite[Lemma~4.10]{buskulic2023convergenceJournal} stay the same. Furthermore, since $R$ also remains identical in both cases, we we can directly get from the original proof that
    \[
    R \geq C_1\pa{\frac{k}{n}}^{1/4}
    \]
    whenever $k \gtrsim n$, $C_1$ being a positive constant that depends only on $B$, $\Cphi$, $\Cphid$ and $D$.

    Concerning $R'$, we first need to adjust the result from~\cite[Lemma~4.9]{buskulic2023convergenceJournal} to our linear operator which gives us that
    \begin{align}\label{eq:init_error_linear}
        \norm{\yv(0) - \yv} \leq C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}} ,
    \end{align}
    with probability at least $1 - d^{-1}$, where $C$ is a constant that depends only on $B$, $\Cphi$, and $D$. From here we follow the original proof and get that by using the descent lemma in~\cite[Lemma~2.64]{BauschkeBook}
    \[
    \lossyzy \leq \max_{\vv \in [\yv,\yvz]}\frac{\norm{\nabla \lossy(\vv)}}{\norm{\vv-\yv}} \frac{\norm{\yvz-\yv}^2}{2} .
    \] 
    Combining this with~\eqref{eq:init_error_linear} and that
    \[
    [\yv,\yvz] \subset \Ball(0,\norm{\yv}+\norm{\yvz}) 
    \]
    allows us to obtain that with probability at least $1 - d^{-1}$ we have
    \[
    \lossyzy \leq \frac{\LLz}{2}\pa{C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}}}^2 .
    \] 
    Lastly using the union bound with the fact that $\psi$ is increasing we obtain that~\eqref{eq:bndR2} is reached with probability at least $1-2n\inv - d\inv$ when
    \begin{equation}\label{eq:R'Rbnd}
    \frac{16}{\sigminA\sqrt{\Cphi^2 + \Cphid^2}}\psi\pa{\frac{\LLz}{2}\pa{C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}}}^2} < C_1\pa{\frac{k}{n}}^{1/4} ,
    \end{equation}
    which leads to the claim of the corollary.
\end{proof}

==> tex/sec_discrete_copy.tex <==
\section{Guarantees with Gradient Descent}

\subsection{Main Assumptions} 
Throughout this paper, we will work under the following standing assumptions.
\vspace*{0.5em}
% 1. grad_y loss is Lipschitz continuous i.e, A-1
% 2. Loss is KL
% 3. min loss = 0
% 4. Phis is C^1 and Lipschitz
% 5. Theta() is bounded.


\begin{mdframed}
    \begin{assumption}\label{ass:l_smooth}
        $\lossy(\cdot) \in \cC^1(\R^m)$ whose gradient is Lipschitz continuous on the bounded sets of~$\R^m$. %\vspace*{-.75em}
    \end{assumption}
    \begin{assumption}\label{ass:l_kl}
        $\lossy(\cdot) \in\KLpsi(\lossy(\yvz)+\eta)$ for some $\eta > 0$. 
    \end{assumption}
    \begin{assumption}\label{ass:min_l_zero}
        $\min \lossy(\cdot) = 0$.
    \end{assumption}
    \begin{assumption}\label{ass:phi_diff}
        $\phi \in \cC^1(\R)$ and $\exists B > 0$ such that $\sup_{x \in \R}|\phi'(x)| \leq B$ and $\phi'$ is $B$-Lipschitz continuous.
    \end{assumption}
    \begin{assumption}\label{ass:theta_bounded}
        $\thetav(\cdot)$ lies in a bounded set of $\R^p$.
    \end{assumption}
    
    % \begin{assumption}\label{ass:nablaL_F}
    % $\exists \Theta \subset \R^p$ large enough such that $\nabla_{\vv}\lossy(\vv) \in \ran{\Jf(\xv)}$ for any $\vv=\fopnl(\xv)$ with $\xv \in \Sigma_\Theta$. 
    % \end{assumption}
\end{mdframed}

\medskip

We now discuss the effects of each of these assumptions. \ref{ass:l_smooth} is used to ensure that the gradient w.r.t $\yvtau$ is informative in a neighborhood around a point which is used to show that~\eqref{eq:grad_descent} is a descent. \ref{ass:l_kl} is necessary to have a sharp loss function up to a reparametrization. Interestingly, the convexity of the loss is not required for some of the guarantees (see the theorem thereafter). \ref{ass:min_l_zero} is natural but easy to relax. \ref{ass:phi_diff} ensures that $\gv(\uv,\cdot)$ is $\cC^1(\R^p;\R^p)$ with a Lipschitz continuous Jacobian on bounded sets. This assumption is met by many usual activation functions such as softmax, sigmoid or hyperbolic tangent. Finally,~\ref{ass:theta_bounded} is classical in convergence proofs of gradient descent and permit to use the Lipschitz property over bounded sets of the loss and the Jacobian of the network to show convergence of gradient descent.


% \begin{mdframed}[frametitle={Assumption on the forward operator}]
%     \begin{assumption}\label{ass:F_diff}
%         $\fopnl \in \cC^1(\R^n;\R^m)$ whose Jacobian $\Jf$ is Lipschitz continuous on the bounded sets of~$\R^n$.
%     \end{assumption}
% \end{mdframed}

\medskip

\subsection{Deterministic Results}

% Until now we provided results in the continuous gradient flow case, however in practice one has to use the discrete version of the algorithm, that is gradient descent. In this discrete version we consider update of the form
% \begin{align}\label{eq:grad_descent}
%     \thetav(\tau+1) = \thetav(\tau) - \gamma \nabla_{\thetavtau}\lossy(\yvtau)
% \end{align}
% where $\gamma$ is the chosen time step. If one chooses gamma infinitely small, it would become equivalent to the gradient flow equation~\eqref{eq:gradflow}. The question is then how should one choose $\gamma$ to ensure that all the results we found in Theorem~\ref{thm:main} remain valid. 

% As a first approach to this discrete problem, we choose a simpler setting than the one of Theorem~\ref{thm:main}. We restrict ourselves to linear problems with forward operator $\fop\in\R^{m\times n}$ and we optimize the network using the MSE loss that is $\loss(\yv(\cdot)) = \norm{\yv(\cdot) - \yv}^2$. This implies that from the assumptions of Theorem~\ref{thm:main} we only need~\ref{ass:phi_diff} and that $\yv \in \ran{\fop}$ to reach the same set of assumptions. Indeed all the assumptions on the loss are met by the MSE and a linear operator obviously respects~\ref{ass:F_diff}.

% We now have everything in place to present the results one can reach in the discrete setting:

We can now state our theorem for gradient descent optimization
% Define the theorem
\begin{theorem}\label{thm:main_discr}
    Consider a network $\gv(\uv,\cdot)$, a forward operator $\fop$ and a loss $\loss$ such that~\ref{ass:l_smooth} to~\ref{ass:theta_bounded} hold. 
    Let $\thetav(\cdot)$ be the parameters found at each iteration of \eqref{eq:grad_descent} where the initialization $\thetavz$ is such that
    \begin{equation}\label{eq:bndR2}
        \sigminjgz > 0 \qandq R' < R
    \end{equation}
    where R' and R obey
    \begin{equation}\label{eq:RandR'2}
        R' = \frac{8}{\sigminA\sigminjgz}\psi(\lossyzy) \qandq R = \frac{\sigminjgz}{2\Lip_{\Ball(\thetavz,R)}(\Jg)}. 
    \end{equation}
    If $\gamma \leq \frac{1}{L}$ with $L = \Lip_{\Ball(\thetavz,R')}(\nabla_\yv\lossy) \Lip_{\Ball(\thetavz,R')}(\Jg)\Lip_{\Ball(\thetavz,R')}(\gv) \norm{\fop}^2$, then the following holds:
\begin{enumerate}[label=(\roman*)]
\item \label{thm:main_y_bounded2} the loss converges to $0$ at the rate
\begin{align}\label{eq:lossrate2}
    \lossytauy &\leq \Psi\inv\left(\xi(\tau)\right)
\end{align}
with $\Psi$ a primitive of $-\psi^2$ and $\xi(\tau) = \eta\frac{\sigminA^2\sigminjgz^2}{16}\tau + \Psi(\lossyzy)$ where $\eta = \gamma - \frac{L\gamma^2}{2} \in [0,\frac{1}{2L}]$. Moreover, $\thetav(\tau)$ converges to a global minimizer $\thetav_{\infty}$ of $\lossy(\fop\gv(\uv,\cdot))$, at the rate
\begin{align}\label{eq:thetarate2}
\norm{\thetav(\tau) - \thetav_{\infty}} &\leq \frac{8}{\sigminjgz\sigminA}\psi\left( \Psi\inv(\xi(\tau)) \right).
\end{align}


\item If $\Argmin(\lossy(\cdot)) = \ens{\yv}$, then $\lim_{\tau \to +\infty}\yv(\tau)=\yv$. In addition, if $\loss$ is convex then
\begin{align}\label{eq:yrate}
\norm{\yvtau - \yvc} \leq 2\norm{\veps} \quad \text{when} \quad \tau\geq \frac{16\Psi(\psi\inv(\norm{\veps}))}{\sigminA^2\sigminjgz^2}-\Psi(\lossy(\yvz)).
\end{align}

\item Assume that $\Argmin(\lossy(\cdot))=\{\yv\}$, that $\loss$ is convex and that
\begin{assumption}\label{ass:A_inj}
$\ker{(\fop)} \cap T_{\Sigma'}(\xvc_{\Sigma'}) = \{0\}$ with $\Sigma'\eqdef \Sigma_{\Ball_{R' + \norm{\thetavz}}}$
%$\lmin(\fop;T_{\Sigma'}(\xvcsigma)) >0$.
\end{assumption}
Then,
\begin{align}\label{eq:xrate_discr}
\norm{\xv(\tau) - \xvc} &\leq \frac{\psi\pa{\Psi\inv\pa{\xi(\tau)}}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))} \nonumber\\
&+ \pa{1+\frac{\norm{\fop}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))}}\dist(\xvc,\Sigma') + \frac{\norm{\veps}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))}.
\end{align}

\end{enumerate}
\end{theorem}

\subsection{Discussion and Consequences}
% discussion Th

% Say that we basically obtain the same thing and now more in depth of the changes that happened.
The main observation from this Theorem is that the guarantees obtained through gradient flow in~\cite{buskulic2023convergenceJournal} hold, up to positive constants, when one uses gradient descent with small enough steps. This constraint on the step size given by $\gamma \leq 1/L$ is very classical when using descent lemmas, where $L$ represent the Lipschitz constant of the gradient of the loss w.r.t the parameters $\thetav$, giving information on the size of the neighborhood around a point where the information of the gradient is relevant. We can now have a more in-depth look at the changes brought by the discretization of the gradient flow.

First, the condition on the non-degenerate initialization given by $R'<R$ stays very similar as only $R'$ changes with a factor 4. The underlying idea that the initialisation should be in a convergence basin of a minimizer stays true. Second, the optimization will also converge to a zero-loss solution at a rate dictated by the application of $\Psi\inv$ on an affine function of time. The change appears in the affine function $\xi(\tau)$ where a factor $\eta/4$ needs to be taken into consideration with eta dependant on the smoothness $L$ described above. This discretization cost in $\xi(\tau)$ comes from lower bounding the value that $\psi'$ could take between two consecutive steps of optimization which we do not need to do in the continuous case. In the theorem, we chose to use a bound that would work for any $\gamma\leq1/L$ but if one know that $\gamma = \lambda/L$ with $\lambda\in ]0,1]$, then the discretization error becomes $\frac{\eta}{(1+\lambda)^2} = \frac{2\lambda - \lambda ^2}{2L(1+\lambda)^2}$. This value is maximized when $\lambda = 1/2$, and since $\Psi\inv$ is strictly decreasing, it provides the best value to minimize the upper bound on the loss.

Choosing the step size in such fashion has other consequences. The first one is that the bigger the step size, the worst the constant on $R'$ with the worst case being given in the theorem to account for all cases. In the limit where $\gamma$ tends to zero, we would have that the constant of $R'$ would be 2 which is what has been found in the gradient flow theorem of~\cite{buskulic2023convergenceJournal}. The other impact would of the step size is on the convergence bound of $\thetav$ where the constant factor would also be lower as gamma goes to zero. As such, there is a trade-off between the speed of the convergence and the requirements on the condition given by $R'$. In more practical cases, one would certainly only have guarantees of the form $\gamma \leq 1/L$ which is what our theorem answers to.

Finally, the convergence in the signal space of $\xv(\tau)$ does not change fundamentally. Indeed, one still requires a restricted injectivity constraint, and the errors due to the noise of the problem and the one due to the choice of model have no reason to change. The only thing that is modified is the convergence rate to the solution as it needs to match the convergence of the loss discussed before. In essence, the finding of~\cite[Theorem 3.2]{buskulic2023convergenceJournal} and all the discussion that followed still hold when one uses gradient descent with a controlled step size that depends on the problem at hand.


%Corollaire probabiliste
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Probabilistic Corollary For a Two-Layer DIP Network}\label{sec:dip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Intro sur l'extension du théorème correspondant + explication DIP + présentation du réseau
% hypothèses et notations
% Corollaire
% Discussion rapide
% Rajouter preuve à la fin

% intro :
The next step is to try to understand when does a network reach the conditions of Theorem~\ref{thm:main_discr} and thus when does it benefit from its recovery guarantees. In the gradient flow case, this question is answered by~\cite[Theorem 4.1]{buskulic2023convergenceJournal} for a two-layer network in the DIP setting. That is, the input $\uv$ is chosen at random and fixed during training while the network learns to transform it into a signal that matches $\yv$. The theorem gives an overparametrization bound under which the network will follow the convergence and recovery guarantees with high probability. We provide the corollary of the theorem that is adapted to gradient descent and where a network obeys the guarantees of~\ref{thm:main_discr} with high probability.

In this section, we consider the two-layer network defined as
\begin{align}\label{eq:dipntk}
    \gdip = \frac{1}{\sqrt{k}}\Vv\phi(\Wv\uv)
\end{align}
with  $\Vv \in \R^{n \times k}$ and $\Wv \in \R^{k \times d}$, and $\phi$ an element-wise nonlinear activation function. In this setting, $k$ is the number of neurons on the hidden layer and the scaling by $\sqrt{k}$ is necessary to control the Jacobian of the network. In the following, we set $\Cphi = \sqrt{\Expect{X\sim\stddistrib}{\phi(X)^2}}$ and $\Cphid = \sqrt{\Expect{X\sim\stddistrib}{\phi'(X)^2}}$.  We will need the following assumptions:


\begin{mdframed}[frametitle={Assumptions on the network input and intialization}]
%\begin{assumption}\label{ass:surjective_op}
%$\fop$ is a surjective linear operator; \vspace*{-.75em}
%\end{assumption}
\begin{assumption}\label{ass:u_sphere}
$\uv$ is a uniform vector on $\sph^{d-1}$;% \vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:w_init}
$\Wv(0)$ has iid entries from $\stddistrib$ and $\Cphi, \Cphid < +\infty$; %\vspace*{-.75em}
\end{assumption}
\begin{assumption}\label{ass:v_init}
$\Vv(0)$ is independent from $\Wv(0)$ and $\uv$ and has iid columns with identity covariance and $D$-bounded centered entries.%\vspace*{-.75em}
\end{assumption}
% \begin{assumption}\label{ass:phi_diff}
% $\phi$ is a twice differentiable function with $B$-bounded derivatives.
% \end{assumption}
% \begin{assumption}\label{ass:phi_lip}
% Both $\phi$ and $\phi'$ are $B$-Lipschitz, for some $B > 0$.
% \end{assumption}
\end{mdframed}

Our main result gives a bound on the level of overparametrization which is sufficient for \eqref{eq:bndR2} to hold. 

\begin{corollary}\label{cor:dip_two_layers_converge_discr}
Suppose that assumptions \ref{ass:l_smooth}, \ref{ass:min_l_zero} and \ref{ass:phi_diff} hold. Let $C$, $C'$ two positive constants that depend only on the activation function and $D$. Let:
\[
\LLz = \max_{\vv \in \Ball\pa{0,C\norm{\fop}\sqrt{n\log(d)}+\sqrt{m}\pa{\norminf{\fop\xvc}+\norminf{\veps}}}} \frac{\norm{\nabla_\vv \lossy(\vv)}}{\norm{\vv-\yv}}.
\]
Consider the one-hidden layer network \eqref{eq:dipntk} where both layers are trained with the initialization satisfying \ref{ass:u_sphere} to \ref{ass:v_init} and the architecture parameters obeying
\begin{align*}
k \geq C' \sigminA^{-4} n \psi\pa{\frac{\LLz}{2}\pa{C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}}}^2}^4 .
%k \geq C \kappa(\fop)^2n \pa{\sqrt{n}\pa{\sqrt{\log(d)} + 1} + \sqrt{m}}^2 .
%k \geq C_1 \kappa(\fop)^2 n^{5/2}m 
\end{align*}
Then \eqref{eq:bndR2} holds with probability at least $1 - 2n^{-1} - d^{-1}$.
\end{corollary}

% Dans la discussion :
% Discuter de gamma qui va dépendre de sqrt(k/n) et de R' donc de l'initialisation du réseau.
% 



As expected, since the variables in Theorem~\ref{thm:main_discr} only change by a constant factor compared to the gradient flow case, the overparametrization bound that we found for the gradient descent case only change by a constant factor compared to the bound found in the gradient flow case. We presented our results with a linear forward operator but if one chooses to use a nonlinear operator, the results from~\cite[Theorem 4.1]{buskulic2023convergenceJournal} will hold when one uses gradient descent as the change is absorbed in the constants.

This corollary only ensures that~\eqref{eq:bndR2} hold with high probability and while it is enough when using gradient flow to obtain convergence and recovery guarantees, it is not the case when using gradient descent. One still needs to ensure that the size of the descent steps $\gamma$ is well chosen to be lower than $\frac{1}{L}$ with $L$ the Lipschitz constant of the gradient of the loss w.r.t $\thetav$. Here the overparametrization of the network will be of help as $L$ depends on $\Lip_{\Ball(\thetavz,R')}(\Jg)\Lip_{\Ball(\thetavz,R')}(\gv)$. first of, by~\cite[Lemma 4.10]{buskulic2023convergenceJournal}, $\Lip_{\Ball(\thetavz,R')}(\Jg)$ is proportional to $\sqrt{n/k}$ and $R'$. Furthermore, if one chooses a bounded $\phi$ or only train the parameters $\Wv$ and fix $\Vv$, then $\Lip_{\Ball(\thetavz,R')}(\gv)$ will also be of order $\sqrt{n/k}$ by~\cite[Theorem 5.39]{vershynin_introduction_2012}.
This means that $\gamma$ is dependent on both the initial solution of the network (via $R'$) and the level of overparametrization (via $k$). The consequence is that very overparametrized networks can use larger descent steps and still benefit from the convergence guarantees previously described.

We can use the case of the Means Square Error (MSE) to see how $\gamma$ evolves with the overparametrization. For that loss function, $\Lip(\nabla_\yv\lossy) = 2$ which means that $\gamma \leq 2 \Lip_{\Ball(\thetavz,R')}(\Jg)\Lip_{\Ball(\thetavz,R')}(\gv) \norm{\fop}^2 \lesssim\frac{k}{nR'\norm{\fop}^2}$. Furthermore, for the MSE, $\psi$ is the square root which means that the bound given in the corollary gives that one needs $k\gtrsim \kappa(\fop)^4n^3m^2$. So by following this overparametrization bound, we already get that one can use $\gamma \lesssim \frac{\norm{\fop}^2n^2m^2}{R'\sigminA^4}$ which for sufficiently high dimensional problem will be a very large bound given that $\fop$ is well enough conditioned.



% Proof
\section{Proofs}
\subsection{Proof of Theorem~\ref{thm:main_discr}}
We first present useful lemmas that will help us prove the claims from Theorem~\ref{thm:main_discr}.

\begin{lemma}\label{lemma:descent_trajectory}
    Assume that~\ref{ass:l_smooth} and~\ref{ass:phi_diff} hold. Let $\thetav(\cdot)$ be a trajectory of~\eqref{eq:grad_descent} and let us assume that $\thetav(\cdot) \in \Omega$ a bounded set of $\R^p$. Then there exists a positive constant $L'$ such that choosing $\gamma \leq 1/L$ with $L = L' \Lip_\Omega(\Jg) \Lip_\Omega(\gv) \norm{\fop}^2$ ensures that $\lossy(\cdot)$ is nonincreasing and thus converges. 
\end{lemma}
\begin{proof}
    We will use similar steps as in classical descent lemmas of gradient descent. First of, let us define $\tau_\delta = \tau + \delta$ with $\delta \in [0,1]$. Then, we extend the definition of~\eqref{eq:grad_descent} such that
    \begin{align*}
        \thetav(\tau_\delta) = \thetavtau - \delta\gamma\nabla_{\thetav}\lossytauy = \thetavtau + \delta(\thetavtauplus - \thetavtau).
    \end{align*}
    We can now use this and the fundamental theorem of calculus to obtain
    \begin{align*}
        \lossy(\yv(\tau+1)) - \lossytauy &= \int_{\tau}^{\tau+1} \nabla_{s}\lossy(\yv(s))\tp ds\\
        &= \int_{0}^{1} \nabla_{\thetav}\lossy(\yv(\tau_\delta))\tp \nabla_{\delta}\thetav(\tau_\delta)\tp d\delta\\
        &= \int_{0}^{1} \nabla_{\thetav}\lossy(\yv(\tau_\delta))\tp (\thetavtauplus - \thetavtau) d\delta.
    \end{align*}
    By substracting a constant and taking the absolute value we have
    \begin{align}\label{eq:descent_lemma_inter}
        \lvert\lossy(\yv(\tau+1)) - &\lossytauy - \nabla_{\thetav}\lossy(\yv(\tau))\tp (\thetavtauplus - \thetavtau)\rvert \nonumber \\
        &= \abs{\int_{0}^{1} (\nabla_{\thetav}\lossy(\yv(\tau_\delta)) - \nabla_{\thetav}\lossy(\yv(\tau)))\tp (\thetavtauplus - \thetavtau) d\delta}\nonumber\\
        &\leq \int_{0}^{1} \norm{\nabla_{\thetav}\lossy(\yv(\tau_\delta)) - \nabla_{\thetav}\lossy(\yv(\tau))} d\delta \norm{\thetavtauplus - \thetavtau}.
    \end{align}
    From here, it is also straightforward that
    \begin{align}
        \nabla_{\thetav}\lossytauy\tp = \fop \Jg(\thetavtau) \nabla_{\yv}\lossytauy.
    \end{align}
    By assumption of the Lemma, we have that $\thetav(\cdot)\in\Omega$, a bounded set of $\R^p$, which also means that by continuity of $\fop$ and $\gv$, $\yv(\cdot)$ lies in a bounded set of $\R^m$. \ref{ass:l_smooth} and the boundedness of $\yv(\cdot)$ indicates that $\nabla_\yv \lossytauy$ is Lipschitz-continuous, and we define its Lipschitz constant as $L'$. This gives us that
    \begin{align}\label{eq:l_smooth_theta_inter}
        \norm{\nabla_{\thetav}\lossy(\yv(\tau_\delta)) - \nabla_{\thetav}\lossy(\yv(\tau))} &\leq \norm{\fop} \Lip_\Omega(\Jg) L' \norm{\yv(\tau_\delta) - \yvtau}\nonumber\\
        &\leq \norm{\fop}^2\Lip_\Omega(\Jg) L' \norm{\gv(\cdot,\thetav(\tau_\delta)) - \gv(\cdot,\thetavtau)}
    \end{align}
    By using once again the fundamental theorem of calculus, we get
    \begin{align*}
        \gv(\cdot,\thetav(\tau_\delta)) - \gv(\cdot,\thetavtau) &= \int_0^\delta \nabla_{\thetav}\gv(\cdot,\thetav(\tau+s))\tp (\thetavtauplus - \thetavtau)ds \\
        &= \int_0^\delta \Jg(\thetav(\tau+s)) (\thetavtauplus - \thetavtau)ds.
    \end{align*}
    Taking the norm gives us 
    \begin{align*}
        \norm{\gv(\cdot,\thetav(\tau_\delta)) - \gv(\cdot,\thetavtau)} &\leq \int_0^\delta \norm{\Jg(\thetav(\tau+s))}ds \norm{(\thetavtauplus - \thetavtau)}\\
        &\leq \delta\Lip_\Omega(\gv)\norm{(\thetavtauplus - \thetavtau)}.
    \end{align*}
    Combining this result with~\eqref{eq:l_smooth_theta_inter} we obtain that  
    \begin{align*}
         \norm{\nabla_{\thetav}\lossy(\yv(\tau_\delta)) - \nabla_{\thetav}\lossy(\yv(\tau))} &\leq \norm{\fop}^2\Lip_\Omega(\Jg) \Lip_\Omega(\gv) L' \norm{\thetavtauplus - \thetavtau}\\
         &\leq L\norm{\thetavtauplus - \thetavtau}.
    \end{align*}
    Going back to~\eqref{eq:descent_lemma_inter} gives us
    \begin{align*}
        \lvert\lossy(\yv(\tau+1)) - &\lossytauy - \nabla_{\thetav}\lossy(\yv(\tau))\tp (\thetavtauplus - \thetavtau)\rvert \nonumber \\
        &\leq \int_{0}^{1} L\norm{\thetavtauplus - \thetavtau}d\delta \norm{\thetavtauplus - \thetavtau}\\
        &\leq \int_{0}^{1} L\delta d\delta \norm{\thetavtauplus - \thetavtau}^2\\
        &\leq \frac{L}{2} \norm{\thetavtauplus - \thetavtau}^2.
    \end{align*}
    We can now recall that $\thetavtauplus - \thetavtau = - \gamma\nabla_{\thetav}\lossytauy$ to conclude that
    \begin{align*}
        \lossy(\yv(\tau+1)) - \lossytauy + \gamma\norm{\nabla_{\thetav}\lossytauy}^2 \leq \frac{L\gamma^2}{2}\norm{\nabla_{\thetav}\lossytauy}^2 \nonumber\\
        \lossy(\yv(\tau+1)) - \lossytauy \leq (\frac{L\gamma^2}{2} - \gamma)\norm{\nabla_{\thetav}\lossytauy}^2.
    \end{align*}
    Now, as long as one chooses $\gamma\leq1/L$,
    \begin{align}\label{eq:descent_size}
        \lossy(\yv(\tau+1)) - \lossytauy \leq - \eta\norm{\nabla_{\thetav}\lossytauy}^2,
    \end{align}
    with $\eta = \gamma - \frac{L\gamma^2}{2} \in [0,\frac{1}{2L}]$, showing that for sufficiently small $\gamma$,~\eqref{eq:grad_descent} is indeed a descent and $\lossy(\yv(\cdot))$ is non-increasing. 
\end{proof}

\begin{lemma}\label{lemma:link_params_singvals_discr}
Assume \ref{ass:l_smooth} to \ref{ass:theta_bounded} hold. Recall $R$ and $R'$ from \eqref{eq:RandR'2}. Let $\thetav(\cdot)$ be a solution of \eqref{eq:grad_descent}.
    \begin{enumerate}[label=(\roman*)]
        \item \label{claim:singvals_bounded_if_params_bounded_discr} If $\thetav \in \Ball(\thetavz,R)$ then
        \begin{align*}
            \sigmin(\jtheta) \geq \sigminjgz/2.
        \end{align*}
        
        \item  \label{claim:params_bounded_if_singvals_bounded_discr} Assume that $\gamma = 1/L$ with $L=\Lip_{\Ball(\thetavz,R')}(\nabla_{\yv}\lossy(\cdot)) \Lip_{\Ball(\thetavz,R')}(\Jg) \Lip_{\Ball(\thetavz,R')}(\gv) \norm{\fop}^2$. Also assume that for all $s\in \{0,\dots,\tau\}$, $\sigminjgs \geq \frac{\sigminjgz}{2}$. Then
        \begin{align*}
            \thetavtau \in \Ball(\thetavz,R').
        \end{align*}
        
        \item \label{claim:sigval_bounded_everywhere_discr}
        If $R'<R$, then for all $t \geq 0$, $\sigminjgt \geq \sigminjgz/2$.
\end{enumerate}
\end{lemma}
\begin{proof}
The proof of~\ref{claim:singvals_bounded_if_params_bounded_discr} and~\ref{claim:sigval_bounded_everywhere_discr} are found in~\cite[Lemma 3.10]{buskulic2023convergenceJournal}. We now prove claim~\ref{claim:params_bounded_if_singvals_bounded_discr}. By~\ref{ass:theta_bounded}, $\thetav(\cdot)$ is bounded which allows us to use Lemma~\ref{lemma:descent_trajectory}. We thus know that there exist an $L$ such that when $\gamma \leq 1/L$, \eqref{eq:grad_descent} will ensures that $\lossy(\yv(\cdot))$ is non-increasing. In order to prove our claim, we use the Lyapunov function
\begin{align}\label{eq:psi_lyapu}
    V(\tau) = \psi(\lossy(\tau)) + \alpha \sum_{i=0}^{\tau  - 1}\norm{\thetav(i+1) - \thetav(i)}
\end{align}
where $\psi$ is the desingularizing function given by the KL property of $\lossy$ (\ref{ass:l_kl}) and $\alpha\in\R^*_+$. Our goal is to show that for a sufficiently small $\alpha$, our Lyapunov function is non-increasing. With that in mind, let us start with the fact that
\begin{align*}
    V(\tau+1) - V(\tau) = \psi(\lossy(\yv(\tau+1))) - \psi(\lossytauy) + \alpha \norm{\thetavtauplus - \thetavtau}.
\end{align*}
Combining~\ref{ass:l_kl} and that $\lossy(\yv(\cdot))$ is non-increasing with our choice of $\gamma$ ensures that our KL property holds for the entire trajectory of \eqref{eq:grad_descent}. By the mean value theorem, we have
\begin{align}\label{eq:mvt_kl}
    \psi(\lossy(\yv(\tau+1))) - \psi(\lossytauy) = \psi'(\lossy(\yv(\tau+\delta)))(\lossy(\yv(\tau+1)) - \lossytauy),
\end{align}
with $\delta\in[0,1]$. Going back to the Lyapunov function and using~\eqref{eq:mvt_kl} and~\eqref{eq:descent_size} we obtain
\begin{align*}
    V(\tau+1) - V(\tau) &\leq  \psi'(\lossy(\yv(\tau+\delta)))(\lossy(\yv(\tau+1)) - \lossytauy) + \alpha \norm{\thetavtauplus - \thetavtau}\\
    &\leq - \psi'(\lossy(\yv(\tau+\delta)))\eta\norm{\nabla_{\thetav}\lossytauy}^2 + \alpha\gamma\norm{\nabla_{\thetav}\lossytauy}\\
    &\leq \norm{\nabla_{\thetav}\lossytauy}\left(\alpha\gamma - \psi'(\lossy(\yv(\tau+\delta)))\eta\norm{\nabla_{\thetav}\lossytauy}\right).
\end{align*}
Our next step is to bound $\psi'(\lossy(\yv(\tau+\delta)))$. We first note by~\ref{ass:theta_bounded} we have that $\thetav(\cdot) \in \Omega$ a bounded set. Then by following the same argument as in Lemma~\ref{lemma:descent_trajectory}, it means that $\yv(\cdot)$ is also bounded which in turns means by~\ref{ass:l_smooth} that $\nabla_{\yv}\lossy(\cdot)$ is Lipschitz with a constant that we call $L'$. Now using the KL property of $\lossy$ we have 
\begin{align}\label{eq:bound_psi_delta}
    \psi'(\lossy(\yv(\tau+\delta))) &\geq \frac{1}{\norm{\nabla_{\yv}\lossy(\yv(\tau+\delta))}} \nonumber\\
    {\small (a)} &\geq \frac{1}{\norm{\nabla_{\yv}\lossytauy}+\norm{\nabla_{\yv}\lossy(\yv(\tau+\delta)) - \nabla_{\yv}\lossytauy}} \nonumber\\
    {\small \ref{ass:l_smooth}} &\geq \frac{1}{\norm{\nabla_{\yv}\lossytauy} + L'\norm{\yv(\tau+\delta) - \yvtau}} \nonumber\\
    &\geq \frac{1}{\norm{\nabla_{\yv}\lossytauy} + L'\norm{\fop}\Lip_\Omega(\Jg)\norm{\thetav(\tau+\delta) - \thetavtau}} \nonumber\\
    &\geq \frac{1}{\norm{\nabla_{\yv}\lossytauy} + L'\norm{\fop}\Lip_\Omega(\Jg)\gamma\delta\norm{\nabla_{\thetav}\lossytauy}} \nonumber\\
    {\small (b)} &\geq \frac{1}{\norm{\nabla_{\yv}\lossytauy}\left(1 + \gamma L'\norm{\fop}^2\Lip_\Omega(\Jg)^2\right)}\nonumber \\
    {\small (c)} &\geq \frac{1}{2\norm{\nabla_{\yv}\lossytauy}}.
\end{align}
In (a) we use a triangular inequality, in (b) the fact that $\delta \leq 1$ and in (c) that $\gamma \leq 1/(L'\norm{\fop}^2\Lip_\Omega(\Jg)^2)$. Going back to our Lyapunov function and combining this last result with the fact that for any $s$, $\sigminjgs \geq \frac{\sigminjgz}{2}$ we get
\begin{align*}
    V(\tau+1) - V(\tau) &\leq \norm{\nabla_{\thetav}\lossytauy}\left(\alpha\gamma - \eta\frac{\norm{\nabla_{\thetav}\lossytauy}}{2\norm{\nabla_{\yv}\lossytauy}}\right)\\
    &\leq \norm{\nabla_{\thetav}\lossytauy}\left(\alpha\gamma - \eta\frac{\sigminjgz\sigminA}{4}\right).
\end{align*}
This shows that as long as $\alpha \leq \frac{\eta \sigminjgz\sigminA}{4\gamma}$, $V(\tau)$ is non-increasing. Since $\gamma \leq 1/L$, we know that $\frac{\eta}{\gamma}\in[1/2,1]$, which means that we can use $\alpha = \frac{\sigminjgz\sigminA}{8}$ to ensure that $V(\tau)$ is non-increasing and thus that $V(\tau)\leq V(0)$. This allows us to obtain that
    \begin{align*}
        \norm{\thetav(\tau) - \thetavz} \leq \sum_{i=0}^{\tau - 1}\norm{\thetav(i+1) - \thetav(i)} \leq \frac{1}{\alpha}\psi(\lossyzy).
    \end{align*}
    This gives us that $\thetav(\cdot) \in \Ball(\thetavz,R')$. It indicates that we can specialise $\gamma$ to match this new bound of $\thetav$. In order to ensure that our results stay true and that our bound holds we are only required to use that $\gamma \leq (\Lip_{\Ball(\thetavz,R')}(\nabla_{\yv}\lossy(\cdot)) \Lip_{\Ball(\thetavz,R')}(\Jg)^2 \norm{\fop}^2)\inv$ which conclude the proof.
    
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:main_discr}]
\begin{enumerate}[label=(\roman*)]
\item We use several energy functions to show our results. We first take as our energy function the loss $\loss$. By Lemma~\ref{lemma:link_params_singvals_discr}~\ref{claim:sigval_bounded_everywhere_discr} and~\eqref{eq:bndR2}, we have that $\sigmin(\Jg(\tau))\geq\sigminjgz/2$. In turn, Lemma~\ref{lemma:link_params_singvals_discr}~\ref{claim:params_bounded_if_singvals_bounded_discr} gives us that $\thetav(\tau) \in \Ball(\thetavz,R')$. With the boundedness of $\thetav$, we can apply classical descent lemma steps and find using Lemma~\ref{lemma:descent_trajectory} with the condition $\gamma\leq1/L$, that the loss is non-increasing w.r.t $\tau$. Embarking from~\eqref{eq:descent_size} and using the bound on $\sigmin(\Jg(\tau))$ we have
\begin{align*}
    \lossy(\yv(\tau+1)) - \lossytauy &\leq -\eta\norm{\nabla_{\thetav}\lossytauy}^2\\ 
    &\leq -\eta\frac{\sigminjgz^2\sigminA^2}{4}\norm{\nabla_{\yv}\lossytauy}^2,
\end{align*}
with $\eta = \gamma - \frac{L\gamma^2}{2} \in [0,\frac{1}{2L}]$. Let $\Psi$ be a primitive of $-\psi'^2$. Then, by the mean value theorem and that $\Psi$ is strictly decreasing we get
\begin{align*}
    \Psi(\lossytauplusy) - \Psi(\lossytauy) &= \Psi'(\lossy(\yv(\tau+\delta)))\left(\lossy(\yv(\tau+1)) - \lossytauy\right)\\
    &= -\psi'(\lossytaudeltay)^2\left(\lossytauplusy - \lossytauy\right)\\
    &\geq \psi'(\lossytaudeltay)^2\eta\frac{\sigminjgz^2\sigminA^2}{4}\norm{\nabla_{\yv}\lossytauy}^2.
\end{align*}
We can use the bound found in~\eqref{eq:bound_psi_delta} to obtain
\begin{align*}
    \Psi(\lossytauplusy) - \Psi(\lossytauy) \geq \eta\frac{\sigminjgz^2\sigminA^2}{16}.
\end{align*}
From this, we use once again that $\Psi$ and $\Psi\inv$ are (strictly) decreasing to see that
\begin{align*}
    \Psi(\lossytauy) - \Psi(\lossyzy) &= \sum_{i=0}^{\tau-1}\Psi(\lossy(\yv(i+1))) - \Psi(\lossy(\yv(i))) \\
    &\geq \tau\eta\frac{\sigminjgz^2\sigminA^2}{16}\\
    \lossytauy &\leq \Psi\inv\left( \tau\eta\frac{\sigminjgz^2\sigminA^2}{16} + \Psi(\lossyzy) \right),
\end{align*}
which gives~\eqref{eq:lossrate2}.

We now know that the loss converges to 0. The next question is the one regarding the convergence of $\thetav$. Because the loss converges and $\thetav$ is bounded, it means that $\thetav$ converges to say $\thetav_\infty$. Going back to the Lyapunov function defined in~\eqref{eq:psi_lyapu} which we know is non--increasing when $\alpha = \sigminjgz\sigminA/8$, we can observe that
\begin{align*}
    V(\infty) - V(\tau) = \psi(\lossy(\yv(\infty))) - \psi(\lossytauy) + \alpha\sum_{i=\tau}^{\infty} \norm{\thetav(i+1) - \thetav(i)} \leq 0.
\end{align*}
Thus, since the loss converges to 0, we get
\begin{align*}
    \norm{\thetavtau - \thetav_\infty} \leq \sum_{i=\tau}^{\infty} \norm{\thetav(i+1) - \thetav(i)} \leq \frac{1}{\alpha}\psi(\lossytauy)
\end{align*}
which proves~\eqref{eq:thetarate2}.

\item We use the same proof as for~\cite[Theorem 3.2 (ii)]{buskulic2023convergenceJournal} and we adapt it to match the new constant in the loss rate.

By continuity of $\fop$ and $\gv(\uv,\cdot)$ we infer that $\yv(\cdot)$ also converges to some value $\y_\infty$. The continuity of $\lossy(\cdot)$ and~\eqref{eq:lossrate2} gives us
\begin{align*}
    0 = \lim_{\tau \to +\infty}\lossytauy = \lossy(\yv_\infty)
\end{align*}
and thus $\yv_\infty \in \Argmin(\lossy)$. Since the latter is the singleton $\{\yv\}$ by assumption we conclude.

In order to obtain the early stopping bound, we use~\cite[Theorem~5]{bolte2017error} that links the KL property of $\lossy(\cdot)$ with an error bound. In our case, this reads
\begin{align}\label{eq:klerrbnd}
\dist(\yvt,\Argmin(\lossy)) = \norm{\yvt - \yv} \leq \psi(\lossytauy).
\end{align}
It then follows that
\begin{align*}
    \norm{\yvtau - \yvc} &\leq \norm{\yvtau - \yv} + \norm{\yv - \yvc}\\
    &\leq \psi(\lossytauy) + \norm{\veps}\\
    &\leq \psi\left(\Psi\inv\left(\eta\frac{\sigminF^2\sigminjgt^2}{16}\tau + \Psi(\lossyzy)\right)\right) + \norm{\veps}.
\end{align*}
Using that $\psi$ is increasing and $\Psi$ is decreasing, the first term is bounded by $\norm{\veps}$ for all $t\geq \frac{16\Psi(\psi\inv(\norm{\veps}))}{\sigminF^2\sigminjgz^2}-\Psi(\lossyzy)$.


    \item By lemma~\ref{lemma:link_params_singvals_discr}, we have that $\thetavtau \in \Ball(\thetavz,R')$ and thus that $\xv(\tau) \in \Sigma'$. Moreover,~\ref{ass:A_inj} ensures that $\lmin(\fop;T_{\Sigma'}(\xvcsigma)) > 0$ which allows us to get the following chain of inequalities:
    \begin{align*}
        \norm{\xvtau - \xvc} &\leq \norm{\xvtau - \xvcsigma} + \dist(\xvc,\Sigma')\\
        \text{\small \ref{ass:A_inj}}&\leq \frac{1}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))} \norm{\yvtau - \fop\xvcsigma} + \dist(\xvc,\Sigma')\\
        &\leq \frac{1}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))}\left( \norm{\yvtau - \yv} + \norm{\yv - \fop\xvc} + \norm{\fop(\xvc - \xvcsigma)}  \right)+ \dist(\xvc,\Sigma')\\
        \begin{split}
         {\small \eqref{eq:prob_inv},\eqref{eq:lossrate2},\eqref{eq:klerrbnd}}  &\leq \frac{\psi(\Psi\inv(\xi(\tau)))}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))}+ \frac{\norm{\epsilon}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))}\\
           &\qquad  + \left(\frac{\norm{\fop}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))} + 1\right)\dist(\xvc,\Sigma')
        \end{split}
       % + \frac{\norm{\epsilon}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))} + \left(\frac{\norm{\fop}}{\lmin(\fop;T_{\Sigma'}(\xvcsigma))} + 1\right)\dist(\xvc,\Sigma')
    \end{align*}
    which conclude the proof of~\eqref{eq:xrate_discr}.
\end{enumerate}
\end{proof}

\subsection{Proof of Corollary~\ref{cor:dip_two_layers_converge_discr}}

\begin{proof}
    The only difference between the $R$ and $R'$ from~\eqref{eq:bndR2} and the ones from~\cite[Theorem~3.2]{buskulic2023convergenceJournal} is that $R'$ in our case is multiplied by a constant factor. This allows us to prove this corollary using the same proof structure as the one for~\cite[Theorem~4.1]{buskulic2023convergenceJournal} that we adapt to take the constant in $R'$ into account and the fact that our operator is linear.
    
    Due to the fact that the assumptions of the original Theorem and this corollary are the same, it means that both~\cite[Lemma~4.9]{buskulic2023convergenceJournal} and~\cite[Lemma~4.10]{buskulic2023convergenceJournal} stay the same. Furthermore, since $R$ also remains identical in both cases, we we can directly get from the original proof that
    \[
    R \geq C_1\pa{\frac{k}{n}}^{1/4}
    \]
    whenever $k \gtrsim n$, $C_1$ being a positive constant that depends only on $B$, $\Cphi$, $\Cphid$ and $D$.

    Concerning $R'$, we first need to adjust the result from~\cite[Lemma~4.9]{buskulic2023convergenceJournal} to our linear operator which gives us that
    \begin{align}\label{eq:init_error_linear}
        \norm{\yv(0) - \yv} \leq C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}} ,
    \end{align}
    with probability at least $1 - d^{-1}$, where $C$ is a constant that depends only on $B$, $\Cphi$, and $D$. From here we follow the original proof and get that by using the descent lemma in~\cite[Lemma~2.64]{BauschkeBook}
    \[
    \lossyzy \leq \max_{\vv \in [\yv,\yvz]}\frac{\norm{\nabla \lossy(\vv)}}{\norm{\vv-\yv}} \frac{\norm{\yvz-\yv}^2}{2} .
    \] 
    Combining this with~\eqref{eq:init_error_linear} and that
    \[
    [\yv,\yvz] \subset \Ball(0,\norm{\yv}+\norm{\yvz}) 
    \]
    allows us to obtain that with probability at least $1 - d^{-1}$ we have
    \[
    \lossyzy \leq \frac{\LLz}{2}\pa{C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}}}^2 .
    \] 
    Lastly using the union bound with the fact that $\psi$ is increasing we obtain that~\eqref{eq:bndR2} is reached with probability at least $1-2n\inv - d\inv$ when
    \begin{equation}\label{eq:R'Rbnd}
    \frac{16}{\sigminA\sqrt{\Cphi^2 + \Cphid^2}}\psi\pa{\frac{\LLz}{2}\pa{C\norm{\fop} \sqrt{n\log(d)} + \sqrt{m}\pa{\norminf{\fop\xvc} + \norminf{\veps}}}^2} < C_1\pa{\frac{k}{n}}^{1/4} ,
    \end{equation}
    which leads to the claim of the corollary.
\end{proof}

